A characterization of wreath products where knapsack is decidable

The knapsack problem for groups was introduced by Miasnikov, Nikolaev, and Ushakov. It is defined for each finitely generated group $G$ and takes as input group elements $g_1,\ldots,g_n,g\in G$ and asks whether there are $x_1,\ldots,x_n\ge 0$ with $g_1^{x_1}\cdots g_n^{x_n}=g$. We study the knapsack problem for wreath products $G\wr H$ of groups $G$ and $H$. Our main result is a characterization of those wreath products $G\wr H$ for which the knapsack problem is decidable. The characterization is in terms of decidability properties of the indiviual factors $G$ and $H$. To this end, we introduce two decision problems, the intersection knapsack problem and its restriction, the positive intersection knapsack problem. Moreover, we apply our main result to $H_3(\mathbb{Z})$, the discrete Heisenberg group, and to Baumslag-Solitar groups $\mathsf{BS}(1,q)$ for $q\ge 1$. First, we show that the knapsack problem is undecidable for $G\wr H_3(\mathbb{Z})$ for any $G\ne 1$. This implies that for $G\ne 1$ and for infinite and virtually nilpotent groups $H$, the knapsack problem for $G\wr H$ is decidable if and only if $H$ is virtually abelian and solvability of systems of exponent equations is decidable for $G$. Second, we show that the knapsack problem is decidable for $G\wr\mathsf{BS}(1,q)$ if and only if solvability of systems of exponent equations is decidable for $G$.

==> h3-old.tex <==
%

Define the matrices
\[
	A = \left(\begin{smallmatrix} 1 & 1 & 0 \\ 0 & 1 & 0 \\ 0 & 0 & 1 \end{smallmatrix}\right), ~
	B = \left(\begin{smallmatrix} 1 & 0 & 0 \\ 0 & 1 & 1 \\ 0 & 0 & 1 \end{smallmatrix}\right), ~
	C = \left(\begin{smallmatrix} 1 & 0 & 1 \\ 0 & 1 & 0 \\ 0 & 0 & 1 \end{smallmatrix}\right).
\]
The discrete Heisenberg group $H_3(\Z)$ is generated by $A$ and $B$.
Its center is generated by $C$.
In this section we prove the following result:

\begin{theorem}
	\label{thm:ikp-h3}
	$\KP^+(H_3(\Z))$ is undecidable.
\end{theorem}

In fact, undecidability holds for interval knapsack where
we look for integer solutions, which reduces to standard interval knapsack
(replace a power $g^x$ by $g^x g^{-y}$).
In the following we only use the (weaker) integer variant.
Together with \cref{main-result} this implies \cref{application-heisenberg}.
The proof is an adaption of the undecidability of knapsack
over $H_3(\Z)^d$ for some constant $d \in \N$ \cite{KoenigLohreyZetzsche2015a}.
We reduce from Hilbert's 10th problem
and use the fact that one can express arithmetic in $H_3(\Z)$.

Let $(E,L)$ be a $\KP^+(H_3(\Z))$-instance where $E = e_1 \dots e_n$.
A power $e_i = g_i^{x_i}$ $x$ is called a {\em head power} if $(0,i-1) \in L$.
The variable $x_i$ is called a {\em head variable}.
A relation $R \subseteq \Z^{\mathcal{V}}$ is {\em head definable}
if there exists an interval knapsack instance $(E,L)$ such that
all variables in $\mathcal{V}$ are head variables in $E$
and $R$ is the set of integer solutions of $(E,L)$ restricted to $\mathcal{V}$.

\begin{lemma}\label{lem:arithmetic}
	Let $x,y,z$ be three distinct variables.
	\begin{enumerate}
		\item $\{ \nu \in \Z^{\{x\}} \mid \nu(x) = a \}$ is head definable for all $a \in \Z$.
		\item $\{ \nu \in \Z^{\{x,y\}} \mid \nu(x) = \nu(y) \}$ is head definable.
		\item $\{ \nu \in \Z^{\{x,y,z\}} \mid \nu(x) + \nu(y) = \nu(z) \}$ is head definable.
		\item $\{ \nu \in \Z^{\{x,y,z\}} \mid \nu(x) \cdot \nu(y) = \nu(z) \}$ is head definable.
	\end{enumerate}
\end{lemma}

\begin{lemma}
	\label{lem:sync}
	If $R,S \subseteq \Z^{\mathcal{V}}$ are head definable
	then $R \cap S$ is also head definable.
\end{lemma}


Now we can prove \cref{thm:ikp-h3}.
We reduce from Hilbert's 10th problem:
Given a finite system $\bigwedge_{j=1}^m E_j$ of polynomial equations $E_j$
of the form $x = a$, $x + y = z$, $xy = z$, $x = y$,
it is undecidable whether there exists an integer solution.
By \cref{lem:arithmetic} and \cref{lem:sync}
one can construct an interval knapsack instance over $H_3(\Z)$ which is solvable
if and only if the system of polynomial equations has a solution.


\subparagraph{Alternative presentation} We show undecidability of
$\SAT^+(H_3(\Z))$ by reducing from solvability of Diophantine
equations over natural numbers. Hence, we are given a finite system
$\bigwedge_{j=1}^m E_j$ of equations of the form $x=a$, $z=x+y$, and $z=x+y$.
It is well-known that solvability of such equation systems is undecidable~.
We represent each variable $x$ by a variable $g_x$ over $H$ such that $g_x=C^x$.
Then, expressing $c=a$ is done simply with $g_x=C^a$. Moreover, for $z=x+y$, we use
\[ C^xB^* \cap B^{x'}C^*\cap (BC)^*\ne \emptyset ~~\wedge~~
  B^{x'}C^*\cap C^zB^*\cap C^y (BC)^*\ne \emptyset \] Note that this
can be expressed in $\SAT^+(H_3(\Z))$ if we have variables for $C^x$,
$B^{x'}$, and $C^z$. Since $B$ and $C$ commute and
$B^iC^j=B^{i'}C^{j'}$ is equivalent to $i=i'$ and $j=j'$, the first
conjunct is equivalent to $x=x'$. Similarly, the second conjunct is
equivalent to $z=x+y$. For multiplication, we use:
\[ C^xA^* \cap A^{x'}C^*\cap (AC)^*\ne \emptyset ~~\wedge~~C^yB^* \cap B^{y'}C^*\cap (BC)^*\ne \emptyset \\
~~\wedge~~ A^{x'}B^*(A^{-1})^*\cap B^{y'}C^*\cap C^zB^*\ne\emptyset.\]
The matrices $A$ and $C$ commute and $A^iC^j=A^{i'}C^{j'}$ is equivalent to $i=i'$ and $j=j'$. Therefore, the first and second conjunct express $x'=x$ and $y'=y$. Moreover, since in $H_3(\Z)$,
we have $A^iB^jA^{-i'}B^{-j'}=C^k$ if and only if $i=i'$, $j=j'$, and $k=ij$, the third conjunct expresses $z=x'y'$, hence $z=xy$.
%
%
%
%


